Stabilizing NMPC Approaches for Underactuated Mechanical Systems on the SE(3) Manifold

This paper addresses the motion control problem for underactuated mechanical systems with full attitude control and one translational force input to manage the six degrees of freedom involved in the three-dimensional Euclidean space. These systems are often classified as second-order nonholonomic due to their completely nonintegrable acceleration constraints. To tackle this complex control problem, we propose two nonlinear model predictive control (NMPC) schemes that ensure closed-loop stability and recursive feasibility without terminal conditions. The system dynamics are modeled on the SE(3) manifold for a globally and unique description of rigid body configurations. One NMPC scheme also aims to reduce mission time as an economic criterion. The controllers' effectiveness is validated through numerical experiments on a quadrotor UAV.

==> macros.tex <==

\newcommand{\mbf}[1]{\ensuremath{{\mathbf{#1}}}}
%\newcommand{\mbf}[1]{\ensuremath{{\bm{#1}}}}

%\renewcommand\labelitemi{{\bm{$\cdot$}}}
\renewcommand\labelitemi{{\bm{$\bullet$}}}

\newcommand{\ten}[1]{\ensuremath{{\cdot}10^{#1}}}

% ---------------------------------- System modeling ---------------------------------------------

\newcommand{\frF}{\ensuremath{\mathcal{F}}}
\newcommand{\frI}{\ensuremath{\mathcal{I}}}
\newcommand{\frL}{\ensuremath{\mathcal{L}}}
\newcommand{\frB}{\ensuremath{\mathcal{B}}}
\newcommand{\frC}[1]{\ensuremath{{\mathcal{C}_{#1}}}}
\newcommand{\frA}[1]{\ensuremath{{\mathcal{A}_{#1}}}}
\newcommand{\RIB}{\ensuremath{\mbf{R}^\mathcal{I}_\mathcal{B}}}
\newcommand{\RIL}{\ensuremath{\mbf{R}^\mathcal{I}_\mathcal{L}}}
\newcommand{\RLA}[1]{\ensuremath{\mbf{R}^\mathcal{L}_{\mathcal{A}_{#1}}}}
\newcommand{\RAB}[1]{\ensuremath{\mbf{R}^{\mathcal{A}_{#1}}_\mathcal{B}}}
\newcommand{\RLB}{\ensuremath{\mbf{R}^\mathcal{L}_\mathcal{B}}}
\newcommand{\RBC}[1]{\ensuremath{\mbf{R}^\mathcal{B}_{\mathcal{C}_{#1}}}}
\newcommand{\RBA}[1]{\ensuremath{\mbf{R}^\mathcal{B}_{\mathcal{A}_{#1}}}}
\newcommand{\RAA}[2]{\ensuremath{\mbf{R}^{\mathcal{A}_{#1}}_{\mathcal{A}_{#2}}}}
\newcommand{\RAC}[2]{\ensuremath{\mbf{R}^{\mathcal{A}_{#1}}_{\mathcal{C}_{#2}}}}
\newcommand{\dLB}{\ensuremath{\mbf{d}^\mathcal{L}_\mathcal{B}}}
\newcommand{\dBC}[1]{\ensuremath{\mbf{d}^\mathcal{B}_{\mathcal{C}_{#1}}}}
\newcommand{\dLA}[1]{\ensuremath{\mbf{d}^\mathcal{L}_{\mathcal{A}_{#1}}}}
\newcommand{\dBA}[1]{\ensuremath{\mbf{d}^\mathcal{B}_{\mathcal{A}_{#1}}}}
\newcommand{\dAB}[1]{\ensuremath{\mbf{d}^{\mathcal{A}_{#1}}_{\mathcal{B}}}}
\newcommand{\dAA}[2]{\ensuremath{\mbf{d}^{\mathcal{A}_{#1}}_{\mathcal{A}_{#2}}}}
\newcommand{\dAC}[2]{\ensuremath{\mbf{d}^{\mathcal{A}_{#1}}_{\mathcal{C}_{#2}}}}

\newcommand{\pLL}{\ensuremath{\mbf{p}^\mathcal{L}_\mathcal{L}}}
\newcommand{\pii}[1]{\ensuremath{\mbf{p}^{\mathcal{C}_{#1}}_{\mathcal{C}_{#1}}}}
\newcommand{\pIL}{\ensuremath{\mbf{p}^\mathcal{I}_\mathcal{L}}}
\newcommand{\pIi}[1]{\ensuremath{\mbf{p}^\mathcal{I}_{\mathcal{C}_{#1}}}}
\newcommand{\dpIL}{\ensuremath{\dot{\mbf{p}}^\mathcal{I}_\mathcal{L}}}
\newcommand{\dpIi}[1]{\ensuremath{\dot{\mbf{p}}^\mathcal{I}_{\mathcal{C}_{#1}}}}

\newcommand{\oLL}{\ensuremath{\mbf{o}^\mathcal{L}_\mathcal{L}}}
\newcommand{\oii}[1]{\ensuremath{\mbf{o}^{\mathcal{C}_{#1}}_{\mathcal{C}_#1}}}
\newcommand{\oIL}{\ensuremath{\mbf{o}^\mathcal{I}_\mathcal{L}}}
\newcommand{\oIi}[1]{\ensuremath{\mbf{o}^\mathcal{I}_{\mathcal{C}_#1}}}
\newcommand{\doIL}{\ensuremath{\dot{\mbf{o}}^\mathcal{I}_\mathcal{L}}}
\newcommand{\doIi}[1]{\ensuremath{\dot{\mbf{o}}^\mathcal{I}_{\mathcal{C}_#1}}}

\newcommand{\dxi}{\ensuremath{\dot{\bm{\xi}}}}
\newcommand{\deta}{\ensuremath{\dot{\bm{\eta}}}}
\newcommand{\dgamma}{\ensuremath{\dot{\bm{\gamma}}}}
\newcommand{\gone}{\ensuremath{{\gamma_1}}}
\newcommand{\dgone}{\ensuremath{\dot{\gamma}_1}}
\newcommand{\gtwo}{\ensuremath{{\gamma_2}}}
\newcommand{\dgtwo}{\ensuremath{\dot{\gamma}_2}}
\newcommand{\aR}{\ensuremath{{\alpha_\text{R}}}}
\newcommand{\daR}{\ensuremath{\dot{\alpha}_\text{R}}}
\newcommand{\aL}{\ensuremath{{\alpha_\text{L}}}}
\newcommand{\daL}{\ensuremath{\dot{\alpha}_\text{L}}}

\newcommand{\wIIL}{\ensuremath{\bm{\omega}^\mathcal{I}_{\mathcal{I}\mathcal{L}}}}
\newcommand{\wLIL}{\ensuremath{\bm{\omega}^\mathcal{L}_{\mathcal{I}\mathcal{L}}}}
\newcommand{\wILB}{\ensuremath{\bm{\omega}^\mathcal{I}_{\mathcal{L}\mathcal{B}}}}
\newcommand{\wALA}[1]{\ensuremath{\bm{\omega}^{\mathcal{A}_{#1}}_{\mathcal{L} \mathcal{A}_{#1}}}}
\newcommand{\wBAB}[1]{\ensuremath{\bm{\omega}^\mathcal{B}_{\mathcal{A}_{#1}\mathcal{B}}}}
\newcommand{\wBLB}{\ensuremath{\bm{\omega}^\mathcal{B}_{\mathcal{L}\mathcal{B}}}}
\newcommand{\wBIB}{\ensuremath{\bm{\omega}^\mathcal{B}_{\mathcal{I}\mathcal{B}}}}
\newcommand{\wABA}[1]{\ensuremath{\bm{\omega}^{\mathcal{A}_{#1}}_{\mathcal{B} \mathcal{A}_{#1}}}}
\newcommand{\wiAi}[1]{\ensuremath{\bm{\omega}^{\mathcal{C}_{#1}}_{\mathcal{A}_{#1} \mathcal{C}_{#1}}}}
\newcommand{\wiBi}[1]{\ensuremath{\bm{\omega}^{\mathcal{C}_{#1}}_{\mathcal{B} \mathcal{C}_{#1}}}}
\newcommand{\wIBi}[1]{\ensuremath{\bm{\omega}^\mathcal{I}_{\mathcal{B} \mathcal{C}_{#1}}}}


\newcommand{\mL}{\ensuremath{m_\mathcal{L}}}
\newcommand{\mi}[1]{\ensuremath{m_{#1}}}
\newcommand{\IL}{\ensuremath{\mbf{I}_\mathcal{L}}}
\newcommand{\Ii}[1]{\ensuremath{\mbf{I}_{#1}}}
\newcommand{\Ji}[1]{\ensuremath{\mbf{J}_{#1}}}
\newcommand{\Ei}[1]{\ensuremath{\mbf{E}_{#1}}}
\newcommand{\Di}[1]{\ensuremath{\mbf{D}_{#1}}}

\newcommand{\myhalf}{\ensuremath{\frac{1}{2}}}

\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\dm}{\ensuremath{\mbf{d}_m}}

\newcommand{\Kin}{\ensuremath{\mathcal{K}}}
\newcommand{\KinL}{\ensuremath{\mathcal{K}_\mathcal{L}}}
\newcommand{\Kini}[1]{\ensuremath{\mathcal{K}_{#1}}}
\newcommand{\Pot}{\ensuremath{\mathcal{U}}}
\newcommand{\PotL}{\ensuremath{\mathcal{U}_\mathcal{L}}}
\newcommand{\Poti}[1]{\ensuremath{\mathcal{U}_{#1}}}

\newcommand{\Weta}{\ensuremath{\mbf{W}_{\bm{\eta}}}}
\newcommand{\ay}{\ensuremath{\mbf{a}_y}}
\newcommand{\az}{\ensuremath{\mbf{a}_z}}

%\newcommand{\eye}[1]{\ensuremath{\mathds{I}_{#1\times#1}}}
\newcommand{\eye}[1]{\ensuremath{\mbf{I}_{#1}}}
\newcommand{\eyenoarg}{\ensuremath{\mbf{I}}}
\newcommand{\zeros}[2]{\ensuremath{\bm{0}_{#1\times#2}}}
\newcommand{\ones}[2]{\ensuremath{\bm{1}_{#1\times#2}}}

\newcommand{\ktaub}{\ensuremath{\frac{k_\tau}{b}}}
\newcommand{\lambdaR}{\ensuremath{\lambda}_\text{R}}
\newcommand{\lambdaL}{\ensuremath{\lambda}_\text{L}}

\newcommand{\rR}{\ensuremath{\mbf{r}_\text{R}}}
\newcommand{\rL}{\ensuremath{\mbf{r}_\text{L}}}
\newcommand{\LambdaR}{\ensuremath{\bm{\Lambda}_\text{R}}}
\newcommand{\LambdaL}{\ensuremath{\bm{\Lambda}_\text{L}}}
\newcommand{\GammaR}{\ensuremath{\bm{\Gamma}_\text{R}}}
\newcommand{\GammaL}{\ensuremath{\bm{\Gamma}_\text{L}}}

\newcommand{\Jac}{\ensuremath{\mathcal{\mbf{J}}}}
\newcommand{\GJac}{\ensuremath{\mathcal{\mbf{W}}}}

\newcommand{\gforce}{\ensuremath{\bm{\vartheta}}}

\newcommand{\fR}{\ensuremath{\mbf{f}_\text{R}}}
\newcommand{\fL}{\ensuremath{\mbf{f}_\text{L}}}
\newcommand{\tauaR}{\ensuremath{\bm{\tau}_{\aR}}}
\newcommand{\tauaL}{\ensuremath{\bm{\tau}_{\aL}}}

\newcommand{\infR}{\ensuremath{f_\text{R}}}
\newcommand{\infL}{\ensuremath{f_\text{L}}}
\newcommand{\intauaR}{\ensuremath{\tau_{\aR}}}
\newcommand{\intauaL}{\ensuremath{\tau_{\aL}}}

\newcommand{\setreal}{\ensuremath{\mathbb{R}}}
\newcommand{\setrealmat}[2]{\ensuremath{\mathbb{R}^{#1\times#2}}}
\newcommand{\setrealvec}[1]{\ensuremath{\mathbb{R}^{#1}}}
%\newcommand{\setrealvec}[1]{\ensuremath{\mathbb{R}^{#1}}}

\newcommand{\vex}[1]{\ensuremath{\text{vex}(#1)}}

% -----------------------------------------------------------------------------------------

% -------------------------------------------- Control -------------------------------------------

\newcommand{\rank}[1]{\ensuremath{\text{rank}\left\{ #1 \right\}}}

%\newcommand{\zdomain}{{\scriptsize$\mathcal{Z}$\normalsize}}
\newcommand{\zdomain}{\ensuremath{\varsigma}}
%\newcommand{\zdomain}{\ensuremath{\mathpzc{z}}}
%\newcommand{\trace}[1]{\ensuremath{\text{trace}\{{#1}\}}}
%\newcommand{\trace}[1]{\ensuremath{\text{tr}\left\{{#1}\right\}}}
\newcommand{\trace}[1]{\ensuremath{\text{trace}\left\{{#1}\right\}}}

\newcommand{\Achi}{\ensuremath{\mbf{A}_{\bm{\chi}}}}
\newcommand{\Bchi}{\ensuremath{\mbf{B}_{\bm{\chi}}}}
\newcommand{\Fchi}{\ensuremath{\mbf{F}_{\bm{\chi}}}}

\newcommand{\tildeAchi}{\ensuremath{\tilde{\mbf{A}}_{\bm{\chi}}}}
\newcommand{\tildeHz}{\ensuremath{\tilde{\mbf{H}}_{\mbf{z}}}}

\newcommand{\Dzu}{\ensuremath{\mbf{D}_{\mbf{z}{\mbf{u}}}}}
\newcommand{\Dzd}{\ensuremath{\mbf{D}_{\mbf{z}{\mbf{d}}}}}

% ------------------------------------------------------------------------------------------------


% ----------------------------------------- State estimation ---------------------------------------------

%\newcommand{\intval}[1]{\ensuremath{{{_\llcorner} \negmedspace {#1} \negmedspace {^\urcorner}}}}
%\newcommand{\intval}[1]{\ensuremath{{{_\llcorner} {#1} {^\urcorner}}}}
%\newcommand{\intval}[1]{\ensuremath{{\prescript{}{\llcorner}{#1}{^\urcorner}}}}
%\newcommand{\intval}[1]{\ensuremath{{\tensor*[_{\llcorner}]{#1}{^{\urcorner}}}}}
%\newcommand{\intval}[1]{\ensuremath{{\tensor*[_{\llcorner}^\ulcorner]{#1}{_\lrcorner^\urcorner}}}}
%\newcommand{\intval}[1]{\ensuremath{{{_{\bm{\llcorner}}} {#1} {^{\bm{\urcorner}}}}}}
%\newcommand{\bintval}[2]{\ensuremath{[{#1},\;{#2}]}}
%\newcommand{\bintval}[2]{\ensuremath{[\,{#1},\:{#2}\,]}}
%\newcommand{\bintval}[2]{\ensuremath{\left[{#1},\;{#2}\right]}}
%\newcommand{\lbound}[1]{\ensuremath{\underline{#1}}}
%\newcommand{\lbound}{\ensuremath{\text{L}}}
%\newcommand{\ubound}{\ensuremath{\text{U}}}
%\newcommand{\midpoint}[1]{\ensuremath{\text{mid}\!\left\{{#1}\right\}}}
%\newcommand{\midpoint}[1]{\ensuremath{\text{mid}\!\left({#1}\right)}}
%\newcommand{\midpoint}[1]{\ensuremath{\text{mid}({#1})}}
%\newcommand{\wid}[1]{\ensuremath{\text{wid}\{{#1}\}}}
%\newcommand{\diam}[1]{\ensuremath{\text{diam}\!\left\{{#1}\right\}}}
%\newcommand{\diam}[1]{\ensuremath{\text{diam}\!\left({#1}\right)}}
%\newcommand{\diam}[1]{\ensuremath{\text{diam}({#1})}}

%\newcommand{\setintval}{\ensuremath{\mathbb{I} \mathbb{R}}}
%\newcommand{\setintvalvec}[1]{\ensuremath{\mathbb{I} \setrealvec{#1}}}
%\newcommand{\setintvalmat}[2]{\ensuremath{\mathbb{I} \setrealmat{#1}{#2}}}

\newcommand{\ubox}{\ensuremath{\mathbb{B}}}
\newcommand{\zonotope}{\ensuremath{\mathbb{Z}}}
%\newcommand{\zonotopefamily}{\ensuremath{{\intval{\zonotope}}}}
\newcommand{\zonotopefamily}{\ensuremath{{\zonotope_\intval{}}}}
\newcommand{\strip}{\ensuremath{\mathbb{S}}}

\newcommand{\iextension}[1]{\ensuremath{\square \left( #1 \right) }}
\newcommand{\zinclusion}[1]{\ensuremath{\diamond \{ {#1} \}}}

\newcommand{\xiB}{\ensuremath{{\bm{\xi}_\frB}}}
\newcommand{\zetaB}{\ensuremath{{\bm{\zeta}_\frB}}}
\newcommand{\phiB}{\ensuremath{{\phi_\frB}}}
\newcommand{\thetaB}{\ensuremath{{\theta_\frB}}}
\newcommand{\psiB}{\ensuremath{{\psi_\frB}}}
\newcommand{\etaB}{\ensuremath{{\bm{\eta}_\frB}}}

\newcommand{\atantwo}[1]{\text{arctan2}\left(#1\right)}

\newcommand{\Anu}{\ensuremath{\mbf{A}_{\bm{\nu}}}}
\newcommand{\Bnu}{\ensuremath{\mbf{B}_{\bm{\nu}}}}
\newcommand{\Fnu}{\ensuremath{\mbf{F}_{\bm{\nu}}}}
\newcommand{\Hnu}{\ensuremath{\mbf{H}_{\bm{\nu}}}}

%\newcommand{\expect}[1]{\ensuremath{\mathcal{E}\{#1\}}}
\newcommand{\expect}[1]{\ensuremath{\mathcal{E}\left[#1\right]}}

\newcommand{\setI}{\ensuremath{\mathbb{I}}}

% ------------------------------------------------------------------------------------------------------------

% ---------------------------------------- Formation control -------------------------------------------------

\newcommand{\hamiplusqnoarg}{\ensuremath{\overset{+}{\bm{\mathrm{H}}}_4}}
\newcommand{\haminusqnoarg}{\ensuremath{\overset{-}{\bm{\mathrm{H}}}_4}}
\newcommand{\hamiplusnoarg}{\ensuremath{\overset{+}{\bm{\mathrm{H}}}_8}}
\newcommand{\haminusnoarg}{\ensuremath{\overset{-}{\bm{\mathrm{H}}}_8}}
\newcommand{\hamiplusq}[1]{\ensuremath{\overset{+}{\bm{\mathrm{H}}}_4(#1)}}
\newcommand{\haminusq}[1]{\ensuremath{\overset{-}{\bm{\mathrm{H}}}_4(#1)}}
\newcommand{\hamiplus}[1]{\ensuremath{\overset{+}{\bm{\mathrm{H}}}_8(#1)}}
\newcommand{\haminus}[1]{\ensuremath{\overset{-}{\bm{\mathrm{H}}}_8(#1)}}
\newcommand{\imi}{\ensuremath{\hat{\imath}}}
\newcommand{\imj}{\ensuremath{\hat{\jmath}}}
\newcommand{\imk}{\ensuremath{\hat{k}}}
\newcommand{\deps}{\ensuremath{\varepsilon}}
%\newcommand{\real}[1]{\ensuremath{\mathcal{R}e(#1)}}
\newcommand{\real}[1]{\ensuremath{\text{Re}(#1)}}
%\newcommand{\imag}[1]{\ensuremath{\mathcal{I}m(#1)}}
\newcommand{\imag}[1]{\ensuremath{\text{Im}(#1)}}
%\newcommand{\prim}[1]{\ensuremath{\mathcal{P}(#1)}}
\newcommand{\prim}[1]{\ensuremath{\mathrm{P}(#1)}}
%\newcommand{\dual}[1]{\ensuremath{\mathcal{D}(#1)}}
\newcommand{\dual}[1]{\ensuremath{\mathrm{D}(#1)}}
\newcommand{\dq}[1]{\ensuremath{\underline{#1}}}
\newcommand{\vecfournoarg}{\ensuremath{\bm{\mathrm{vec}}_4}}
\newcommand{\veceightnoarg}{\ensuremath{\bm{\mathrm{vec}}_8}}
\newcommand{\vecfour}[1]{\ensuremath{\bm{\mathrm{vec}}_4(#1)}}
\newcommand{\veceight}[1]{\ensuremath{\bm{\mathrm{vec}}_8(#1)}}

% ------------------------------------------------------------------------------------------------------------


%\newcommand{\setreal}{\ensuremath{\mathbb{R}}}
%\newcommand{\setrealmat}[2]{\ensuremath{\mathbb{R}^{#1\times#2}}}
%\newcommand{\setrealvec}[1]{\ensuremath{\mathbb{R}^{#1}}}
\newcommand{\realset}{\ensuremath{\mathbb{R}}}
\newcommand{\realsetmat}[2]{\ensuremath{\mathbb{R}^{#1\times#2}}}
%\newcommand{\setrealvec}[1]{\ensuremath{\mathbb{R}^{#1}}}
%\newcommand{\setrealvec}[1]{\ensuremath{\mathbb{R}^{#1}}}

%\newcommand{\ninf}[1]{\ensuremath{\|{#1}\|_\infty}}
%\newcommand{\realset}[1]{\ensuremath{\mathbb{R}^{#1}}}
%\newcommand{\intvalset}[1]{\ensuremath{\mathbb{I}\mathbb{R}^{#1}}}
\newcommand{\intvalset}{\ensuremath{\mathbb{I}\mathbb{R}}}
\newcommand{\intvalsetmat}[2]{\ensuremath{\mathbb{I}\mathbb{R}^{#1\times#2}}}
\newcommand{\naturalset}{\ensuremath{\mathbb{N}}}

%\newcommand{\modelset}{\ensuremath{\mathbb{I}}}
\newcommand{\modelset}{\ensuremath{\mathcal{M}}}

\newcommand{\standardcz}{\ensuremath{Z = \left\{ \mbf{G}, \mbf{c}, \mbf{A}, \mbf{b} \right\}}}
\newcommand{\standardib}{\ensuremath{\mathcal{B} = \cup_{j=1}^{n_b} B_{(j)}}}
%\newcommand{\standardref}{\ensuremath{\cup_{j=1}^{n_b} \iextension{\bar{\mbf{f}}(B_j)}}}
%\newcommand{\particularref}{\ensuremath{\cup_{j=1}^{n_b} \iextension{\bar{\mbf{f}}(B_j,\mbf{u}_{k-1})}}}
\newcommand{\standardref}{\ensuremath{\cup_{j=1}^{n_b} \square(\bar{\mbf{f}}(B_{(j)}))}}
\newcommand{\particularref}{\ensuremath{\cup_{j=1}^{n_b} \square(\bar{\mbf{f}}(B_{(j)},\mbf{u}_{k-1}))}}

\newcommand{\intval}[1]{\ensuremath{{\tensor*[_{\llcorner}]{#1}{^{\urcorner}}}}}
\newcommand{\bintval}[2]{\ensuremath{[\,{#1},\:{#2}\,]}}
\newcommand{\lbound}{\ensuremath{\text{L}}}
\newcommand{\ubound}{\ensuremath{\text{U}}}
\newcommand{\midpoint}[1]{\ensuremath{\text{mid}({#1})}}
\newcommand{\wid}[1]{\ensuremath{\text{wid}\{{#1}\}}}
\newcommand{\diam}[1]{\ensuremath{\text{diam}({#1})}}
\newcommand{\rad}[1]{\ensuremath{\text{rad}({#1})}}

\newcommand{\ginter}[1]{\ensuremath{\cap_{\mbf{#1}}}}

\newcommand{\gzinclusion}{\ensuremath{\triangleleft}}

\newcommand{\ninf}[1]{\ensuremath{\|{#1}\|_\infty}}
\newcommand{\none}[1]{\ensuremath{\|{#1}\|_1}}
\newcommand{\ntwo}[1]{\ensuremath{\|{#1}\|_2}}
\newcommand{\conball}{\ensuremath{B_\infty(\mathbf{A},\mathbf{b})}}
\newcommand{\resconball}{\ensuremath{\bar{B}_\infty(\bar{\mathbf{A}},\bar{\mathbf{b}})}}

\newcommand{\xim}{\ensuremath{\bm{\xi}_\text{m}}}
\newcommand{\xir}{\ensuremath{\bm{\xi}_\text{r}}}
\newcommand{\xil}{\ensuremath{\bm{\xi}^\text{L}}}
\newcommand{\xiu}{\ensuremath{\bm{\xi}^\text{U}}}
\newcommand{\betal}{\ensuremath{\bm{\beta}^\text{L}}}
\newcommand{\betau}{\ensuremath{\bm{\beta}^\text{U}}}
%\newcommand{\gammal}{\ensuremath{\bm{\gamma}^\text{L}}}
%\newcommand{\gammau}{\ensuremath{\bm{\gamma}^\text{U}}}	
\newcommand{\zetal}{\ensuremath{\bm{\zeta}^\text{L}}}
\newcommand{\zetau}{\ensuremath{\bm{\zeta}^\text{U}}}

%\newcommand{\arrowmatrix}[3]{\ensuremath{\underset{\xleftrightarrow[\scriptstyle{#2}]{\hphantom{#1}}}{\left[#1\right]}\left.\!\!\vphantom{#1}\right\updownarrow\!{\scriptstyle{#3}}}}
\newcommand{\arrowmatrix}[3]{\ensuremath{\underset{\xrightarrow[\scriptstyle{#2}]{\hphantom{#1}}}{\left[#1\right]}\left.\!\!\vphantom{#1}\right\downarrow\!{\scriptstyle{#3}}}}

\newcommand{\downarrowmatrix}[2]{\ensuremath{{\left[#1\right]}\left.\!\!\vphantom{#1}\right\downarrow\!{\scriptstyle{#2}}}}


\newcommand{\alamobravo}{ZMV}
\newcommand{\combastelbravo}{ZFO}

\newcommand{\dsum}[2]{\ensuremath{{\displaystyle\sum_{#1}^{#2}}}}
\newcommand{\dprod}[2]{\ensuremath{{\displaystyle\prod_{#1}^{#2}}}}


% Text colors
%\definecolor{orange}{RGB}{255,69,0}
\newcommand{\textred}[1]{\textcolor{red}{#1}}
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}
\newcommand{\textgreen}[1]{\textcolor{green}{#1}}
\newcommand{\textoran}[1]{\textcolor{orange}{#1}}
\newcommand{\textpurp}[1]{\textcolor{purple}{#1}}
% Further abbreviations
\newcommand{\tred}[1]{\textred{#1}}
\newcommand{\tblue}[1]{\textblue{#1}}
\newcommand{\tgreen}[1]{\textgreen{#1}}
\newcommand{\toran}[1]{\textoran{#1}}

% Renew commands to remove colors
\renewcommand{\textred}[1]{#1}
\renewcommand{\textblue}[1]{#1}
\renewcommand{\textgreen}[1]{#1}
%\renewcommand{\textoran}[1]{#1}
\renewcommand{\textpurp}[1]{#1}



%\newcommand{\seq}[1]{\ensuremath{{\underset{\rightarrow}{#1}}}}
%\newcommand{\seq}[1]{\ensuremath{{\underset{\longrightarrow}{#1}}}}
\newcommand{\seq}[1]{\ensuremath{{\protect\overset{\to}{#1}}}} % \protect solves issues when using \overset in figure captions
%\newcommand{\seq}[1]{\ensuremath{{\overset{\vspace{-0.5em}\to}{#1}}}}
%\newcommand{\seq}[1]{\ensuremath{{\oset{\to}{#1}}}}
%\newcommand{\seq}[1]{\ensuremath{{\overset{\lower.5em\hbox{\to}}{#1}}}}
%\newcommand{\seq}[1]{\ensuremath{{\overrightarrow{#1}}}}

\newcommand{\zerospace}{\ensuremath{{\,\!}}}
\newcommand{\nspace}{\ensuremath{\zerospace}}
\newcommand{\zspace}{\ensuremath{\zerospace}}
\newcommand{\inv}[1]{\ensuremath{{#1}\zerospace^{-1}}}


\newcommand{\zseq}[1]{\ensuremath{{\protect\overset{\to}{#1}}\zspace}} %

\newcommand{\noarg}{\ensuremath{\_\,}}
\newcommand{\emptyarg}{\noarg}
\newcommand{\etyarg}{\noarg}

\newcommand{\cmrk}{\ensuremath{\checkmark}}


